Less is More: Clustered Cross-Covariance Control for Offline RL

A fundamental challenge in offline reinforcement learning is distributional shift. Scarce data or datasets dominated by out-of-distribution (OOD) areas exacerbate this issue. Our theoretical analysis and experiments show that the standard squared error objective induces a harmful TD cross covariance. This effect amplifies in OOD areas, biasing optimization and degrading policy learning. To counteract this mechanism, we develop two complementary strategies: partitioned buffer sampling that restricts updates to localized replay partitions, attenuates irregular covariance effects, and aligns update directions, yielding a scheme that is easy to integrate with existing implementations, namely Clustered Cross-Covariance Control for TD (C^4). We also introduce an explicit gradient-based corrective penalty that cancels the covariance induced bias within each update. We prove that buffer partitioning preserves the lower bound property of the maximization objective, and that these constraints mitigate excessive conservatism in extreme OOD areas without altering the core behavior of policy constrained offline reinforcement learning. Empirically, our method showcases higher stability and up to 30% improvement in returns over prior methods, especially with small datasets and splits that emphasize OOD areas.

==> Chapter/Sec7_Exp-v1.tex <==

\section{Experimental Results}

In this section, we present experimental studies to assess our proposed method by answering the following questions:
\begin{enumerate}[label=Q\arabic*.]
\item How does it perform on offline RL relative to existing approaches across standard benchmarks, particularly under reduced-data regimes?
\item How is performance influenced by factors such as the number of initial clusters and the quality of the data?
\item Can the plug-and-play method \(C^4\) adapt to different types of algorithms?
\end{enumerate}




\subsection{Implement}
\blue{
We compare our method with Behavior Cloning (BC) and a comprehensive set of state-of-the-art offline reinforcement learning algorithms. First, we consider standard offline RL baselines, including CQL~\citep{kumar2020conservative}, TD3+BC~\citep{fujimoto2021minimalist}, and IQL~\citep{iql}. Next, we evaluate data-efficient algorithms such as DOGE~\citep{li2022data} and TSRL~\citep{cheng2023look}. DOGE is selected for its strong out-of-distribution generalization via state-conditioned distance functions, while TSRL exploits temporal symmetry in system dynamics. Furthermore, we include recent high-performing methods: BPPO~\citep{zhuang2023behavior}, which leverages PPO-based clipping for monotonic improvement, and A2PR~\citep{liu2024adaptive}, which employs adaptive regularization with a VAE-augmented policy.}

\blue{
Additionally, we compare our approach with those that act as plug-and-play regularizers or share similar design philosophies. To address gradient collapse in sparse data regimes, we evaluate LN and DR3~\citep{kumar2022dr3,yue2023understanding}. We also include SORL~\citep{mao2024stylized}, which aligns with our motivation by performing data clustering, though it operates at the trajectory level.}



% \blue{
% Our method is designed to be plug-and-play and can be readily incorporated into numerous existing offline RL frameworks. In the experiments, we instantiate it on top of both CQL and TD3+BC. Unless explicitly stated, CQL serves as the base algorithm, and our method is indicated with the notation \textit{"Ours"}.
% We implement all experiments in PyTorch 2.1.2 on Ubuntu 20.04.4 LTS with four NVIDIA GeForce RTX 3090 GPUs. The actor and critic are ReLU multilayer perceptrons with four hidden layers of width 256. We train with Adam using batch size 256, learning rate $1\times10^{-4}$ for the actor, learning rate $3\times10^{-4}$ for the critic, and discount factor $\gamma=0.99$. Unless stated otherwise we use default hyperparameters $\alpha$ following CQL \citep{kumar2020conservative}. 
% In addition, we instantiate $\nabla_{x} Q_{\psi}(x)$ as the network’s penultimate layer (the learned features), consistent with common RL implementations \citep{kumar2022dr3}.
% % Reported results are averaged over 3 to 5 random seeds.
% We follow the D4RL protocol for normalized scores \footnote{\url{[https://github.com/Farama-Foundation/D4RL/}}. Given a task score, and the corresponding random and expert scores (as reported in Table \ref{table:datasets-overview}), the normalized score is defined as
% $
% \mathrm{normalized\ score}
% =100\times\frac{\mathrm{score}-\mathrm{random\ score}}{\mathrm{expert\ score}-\mathrm{random\ score}}\, .
% $
% Unless noted, we report the mean normalized score over 3 to 5 repetitions per setting.}


\subsection{Main Results}
\blue{
We focus our primary evaluation on the {data-scarce regime}, restricting the D4RL MuJoCo benchmark to only \textbf{10k} state-action pairs per task (approximately 1\% of the full dataset). This setting rigorously tests the generalization limits of offline RL algorithms. As detailed in Table~\ref{table:locomotion}, we benchmark against a wide spectrum of methods, including standard baselines (TD3+BC, CQL, IQL), data-efficient algorithms (DOGE, TSRL), and stronger OOD-aware baselines (BPPO, A2PR). To provide a holistic view, Figure~\ref{fig:locomotion-radar} further contrasts our method with regularization-focused baselines (LN, DR3, SORL). Despite the extreme data sparsity, our approach demonstrates exceptional robustness, recovering nearly 75\% of expert performance. Crucially, it surpasses all competing baselines by an average margin of over \textbf{30\%}, highlighting its superior data efficiency.}

% ---------- Table 1: Locomotion ----------
% \begin{table}[t]
% \centering
% \caption{\small Normalized scores on D4RL MuJoCo locomotion tasks using reduced-size datasets (10k samples). Abbreviations fr, mr, and me denote full-replay, medium-replay, and medium-expert, respectively.}
% \resizebox{\textwidth}{!}{
% \begin{tabular}{lccccccc}
% \toprule
% Task & TD3+BC & BC & CQL & IQL & DOGE & TSRL & Ours \\
% \midrule
% Hopper-m       & 30.7$\pm$13.2 & 28.8$\pm$12.7 & 50.1$\pm$22.3 & 61.0$\pm$6.2  & 55.6$\pm$8.3  & 60.9$\pm$4.1   & \textbf{69.2$\pm$12.7} \\
% Hopper-mr      & 11.3$\pm$4.7  & 19.7$\pm$18.8 & 13.2$\pm$2.0  & 16.2$\pm$3.0  & 19.1$\pm$3.3  & 23.5$\pm$8.8   & \textbf{45.9$\pm$8.4} \\
% Hopper-me      & 22.6$\pm$13.9 & 38.2$\pm$8.7  & 43.2$\pm$6.9  & 51.7$\pm$7.0  & 36.8$\pm$34.5 & 56.6$\pm$13.9  & \textbf{81.3$\pm$6.0} \\
% Hopper-e       & 53.6$\pm$17.1 & 50.3$\pm$9.5  & 56.1$\pm$26.4 & 60.9$\pm$9.6  & 62.2$\pm$21.7 & 76.7$\pm$20.4  & \textbf{107.0$\pm$2.8} \\
% Hopper-fr      & 32.0$\pm$13.5 & 30.5$\pm$12.4 & 45.0$\pm$22.0 & 56.0$\pm$6.3  & 54.0$\pm$8.4  & 53.4$\pm$11.3  & \textbf{65.3$\pm$9.4} \\
% \midrule
% Halfcheetah-m  & 25.9$\pm$8.4  & 40.2$\pm$8.0  & 41.7$\pm$2.2  & 35.6$\pm$2.9  & 42.8$\pm$2.9  & 43.3$\pm$2.8   & \textbf{46.3$\pm$3.1} \\
% Halfcheetah-mr & 29.1$\pm$8.3  & 25.2$\pm$8.8  & 16.3$\pm$4.9  & 34.1$\pm$6.3  & 26.3$\pm$3.1  & 27.7$\pm$3.8   & \textbf{43.1$\pm$5.3} \\
% Halfcheetah-me & 23.5$\pm$13.6 & 33.7$\pm$7.4  & 39.7$\pm$6.4  & 14.3$\pm$7.3  & 33.1$\pm$8.8  & 37.2$\pm$14.9  & \textbf{46.0$\pm$3.5} \\
% Halfcheetah-e  & 26.4$\pm$4.2  & 25.8$\pm$3.4  & 5.8$\pm$1.3   & -1.1$\pm$3.8  & 1.4$\pm$3.1   & 42.0$\pm$26.4  & \textbf{75.8$\pm$5.2} \\
% Halfcheetah-fr & 28.0$\pm$8.6  & 41.0$\pm$8.1  & 45.0$\pm$2.4  & 33.0$\pm$3.0  & 43.0$\pm$3.1  & 41.0$\pm$3.0   & \textbf{58.1$\pm$3.4} \\
% \midrule
% Walker2d-m     & 11.2$\pm$19.2 & 25.4$\pm$8.6  & 54.1$\pm$15.5 & 34.2$\pm$5.2  & 53.7$\pm$12.6 & 47.3$\pm$10.1  & \textbf{65.9$\pm$7.8} \\
% Walker2d-mr    & 9.3$\pm$6.6   & 2.5$\pm$2.8   & 13.8$\pm$5.3  & 17.7$\pm$8.9  & 15.5$\pm$9.2  & 27.6$\pm$12.4  & \textbf{55.4$\pm$5.9} \\
% Walker2d-me    & 12.4$\pm$15.7 & 35.1$\pm$14.4 & 26.0$\pm$14.0 & 38.0$\pm$12.2 & 42.5$\pm$11.4 & 50.9$\pm$26.4  & \textbf{96.3$\pm$10.4} \\
% Walker2d-e     & 29.5$\pm$23.5 & 37.9$\pm$6.3  & 56.0$\pm$29.4 & 16.2$\pm$3.2  & 81.2$\pm$18.6 & 104.9$\pm$10.6 & \textbf{109.5$\pm$0.3} \\
% Walker2d-fr    & 14.2$\pm$19.5 & 26.2$\pm$8.7  & 55.0$\pm$16.0 & 36.0$\pm$5.6  & 55.5$\pm$12.3 & 44.3$\pm$10.4  & \textbf{77.3$\pm$7.1} \\
% \midrule
% Ant-me         & 52.0$\pm$18.2 & 36.0$\pm$9.0  & 74.0$\pm$25.0 & 66.0$\pm$10.5 & 82.0$\pm$16.4 & 83.6$\pm$12.4  & \textbf{100.9$\pm$5.0} \\
% Ant-m          & 46.0$\pm$17.4 & 33.0$\pm$8.2  & 62.0$\pm$22.1 & 56.0$\pm$9.3  & 69.0$\pm$15.2 & 72.2$\pm$10.6  & \textbf{84.5$\pm$6.1} \\
% Ant-mr         & 31.0$\pm$15.5 & 21.0$\pm$7.3  & 36.0$\pm$16.3 & 41.0$\pm$10.8 & 46.0$\pm$12.9 & 49.4$\pm$13.1  & \textbf{65.8$\pm$6.9} \\
% Ant-e          & 72.0$\pm$25.0 & 57.0$\pm$14.2 & 94.0$\pm$29.4 & 82.0$\pm$15.0 & 98.0$\pm$20.3 & 100.7$\pm$12.6 & \textbf{109.6$\pm$2.7} \\
% Ant-fr         & 70.0$\pm$24.0 & 55.0$\pm$9.5  & 92.0$\pm$26.5 & 80.0$\pm$15.0 & 96.0$\pm$20.0 & 99.8$\pm$12.0  & \textbf{107.6$\pm$3.2} \\
% \midrule
% Average        & 31.5          & 33.1          & 46.0          & 41.4          & 50.7          & 57.2           & 75.7 \\
% \bottomrule
% \end{tabular}}
% \label{table:locomotion}
% \end{table}

\begin{table}[t]
\centering
\renewcommand{\arraystretch}{1.1}
\caption{\small Normalized scores on D4RL MuJoCo locomotion tasks using reduced-size datasets (10k samples). Abbreviations fr, mr, and me denote full-replay, medium-replay, and medium-expert, respectively.}
\resizebox{\textwidth}{!}{
\begin{tabular}{lcccccccc}
\toprule
Task & TD3+BC & CQL & IQL & DOGE & BPPO & TSRL & A2PR & Ours \\
\midrule
Hopper-m       & 30.7$\pm$13.2 & 50.1$\pm$22.3 & 61.0$\pm$6.2  & 55.6$\pm$8.3  & 55.0$\pm$7.8   & 60.9$\pm$4.1   & 55.9$\pm$8.4   & \textbf{69.2$\pm$12.7} \\
Hopper-mr      & 11.3$\pm$4.7  & 13.2$\pm$2.0  & 16.2$\pm$3.0  & 19.1$\pm$3.3  & 45.1$\pm$8.7   & 23.5$\pm$8.8   & 12.5$\pm$5.9   & \textbf{45.9$\pm$8.4} \\
Hopper-me      & 22.6$\pm$13.9 & 43.2$\pm$6.9  & 51.7$\pm$7.0  & 36.8$\pm$34.5 & 27.9$\pm$15.2  & 56.6$\pm$13.9  & 49.7$\pm$10.7  & \textbf{81.3$\pm$6.0} \\
Hopper-e       & 53.6$\pm$17.1 & 56.1$\pm$26.4 & 60.9$\pm$9.6  & 62.2$\pm$21.7 & 85.0$\pm$17.9  & 76.7$\pm$20.4  & 80.0$\pm$16.8  & \textbf{107.0$\pm$2.8} \\
Hopper-fr      & 32.0$\pm$13.5 & 45.0$\pm$22.0 & 56.0$\pm$6.3  & 54.0$\pm$8.4  & 60.0$\pm$9.7   & 53.4$\pm$11.3  & 55.0$\pm$8.9   & \textbf{65.3$\pm$9.4} \\
\midrule
Halfcheetah-m  & 25.9$\pm$8.4  & 41.7$\pm$2.2  & 35.6$\pm$2.9  & 42.8$\pm$2.9  & 28.5$\pm$3.2   & 43.3$\pm$2.8   & 37.1$\pm$2.7   & \textbf{46.3$\pm$3.1} \\
Halfcheetah-mr & 29.1$\pm$8.3  & 16.3$\pm$4.9  & 34.1$\pm$6.3  & 26.3$\pm$3.1  & 34.4$\pm$4.2   & 27.7$\pm$3.8   & 23.6$\pm$4.7   & \textbf{43.1$\pm$5.3} \\
Halfcheetah-me & 23.5$\pm$13.6 & 39.7$\pm$6.4  & 14.3$\pm$7.3  & 33.1$\pm$8.8  & 22.3$\pm$9.6   & 37.2$\pm$14.9  & 32.4$\pm$8.3   & \textbf{46.0$\pm$3.5} \\
Halfcheetah-e  & 26.4$\pm$4.2  & 5.8$\pm$1.3   & -1.1$\pm$3.8  & 1.4$\pm$3.1   & 6.5$\pm$3.4    & 42.0$\pm$26.4  & 36.0$\pm$7.8   & \textbf{75.8$\pm$5.2} \\
Halfcheetah-fr & 28.0$\pm$8.6  & 45.0$\pm$2.4  & 33.0$\pm$3.0  & 43.0$\pm$3.1  & 37.0$\pm$3.6   & 41.0$\pm$3.0   & 39.0$\pm$4.1   & \textbf{58.1$\pm$3.4} \\
\midrule
Walker2d-m     & 11.2$\pm$19.2 & 54.1$\pm$15.5 & 34.2$\pm$5.2  & 53.7$\pm$12.6 & 54.7$\pm$11.4  & 47.3$\pm$10.1  & 5.9$\pm$5.2    & \textbf{65.9$\pm$7.8} \\
Walker2d-mr    & 9.3$\pm$6.6   & 13.8$\pm$5.3  & 17.7$\pm$8.9  & 15.5$\pm$9.2  & 29.5$\pm$8.7   & 27.6$\pm$12.4  & 34.4$\pm$8.9   & \textbf{55.4$\pm$5.9} \\
Walker2d-me    & 12.4$\pm$15.7 & 26.0$\pm$14.0 & 38.0$\pm$12.2 & 42.5$\pm$11.4 & 61.3$\pm$12.2  & 50.9$\pm$26.4  & 56.5$\pm$11.5  & \textbf{96.3$\pm$10.4} \\
Walker2d-e     & 29.5$\pm$23.5 & 56.0$\pm$29.4 & 16.2$\pm$3.2  & 81.2$\pm$18.6 & 102.0$\pm$9.7  & 104.9$\pm$10.6 & 98.0$\pm$7.9   & \textbf{109.5$\pm$0.3} \\
Walker2d-fr    & 14.2$\pm$19.5 & 55.0$\pm$16.0 & 36.0$\pm$5.6  & 55.5$\pm$12.3 & 52.0$\pm$10.9  & 44.3$\pm$10.4  & 48.0$\pm$9.6   & \textbf{77.3$\pm$7.1} \\
\midrule
Ant-me         & 52.0$\pm$18.2 & 74.0$\pm$25.0 & 66.0$\pm$10.5 & 82.0$\pm$16.4 & 85.5$\pm$13.7  & 83.6$\pm$12.4  & 66.7$\pm$10.2  & \textbf{100.9$\pm$5.0} \\
Ant-m          & 46.0$\pm$17.4 & 62.0$\pm$22.1 & 56.0$\pm$9.3  & 69.0$\pm$15.2 & 78.0$\pm$11.9  & 72.2$\pm$10.6  & 64.0$\pm$9.3   & \textbf{84.5$\pm$6.1} \\
Ant-mr         & 31.0$\pm$15.5 & 36.0$\pm$16.3 & 41.0$\pm$10.8 & 46.0$\pm$12.9 & 52.0$\pm$10.8  & 49.4$\pm$13.1  & 44.0$\pm$9.1   & \textbf{65.8$\pm$6.9} \\
Ant-e          & 72.0$\pm$25.0 & 94.0$\pm$29.4 & 82.0$\pm$15.0 & 98.0$\pm$20.3 & 103.0$\pm$11.2 & 100.7$\pm$12.6 & 88.0$\pm$10.6  & \textbf{109.6$\pm$2.7} \\
Ant-fr         & 70.0$\pm$24.0 & 92.0$\pm$26.5 & 80.0$\pm$15.0 & 96.0$\pm$20.0 & 102.0$\pm$11.7 & 99.8$\pm$12.0  & 86.0$\pm$10.4  & \textbf{107.6$\pm$3.2} \\
\midrule
Average        & 31.5          & 46.0          & 41.4          & 50.7          & 56.1          & 57.2           & 50.6           & 75.7 \\
\bottomrule
\end{tabular}}
\label{table:locomotion}
\end{table}




% ---------- Figure: Radar Plot ----------
\begin{figure}[h]
  \centering
  \includegraphics[width=\linewidth]{./fig/locomotion/radar.pdf}
  \vspace{-10pt}
  \caption{\small Radar charts comparing normalized scores on D4RL MuJoCo locomotion tasks (10k samples).}
  \label{fig:locomotion-radar}
\end{figure}
\blue{
In addition to performance, we analyze the computational efficiency and hyperparameter sensitivity of our method (Figure~\ref{fig:runtime}). We benchmark wall-clock training times over 300K optimization steps. Incorporating $C^4$ into standard backbones, including CQL and TD3+BC, introduces only moderate overhead. Our method remains highly efficient compared to complex baselines like TSRL and DOGE, while matching the runtime profile of other regularizers, such as LN, DR3 and SORL. Furthermore, sensitivity studies on $\lambda$ and $\alpha$ reveal robust performance across a broad range of parameter values, minimizing the need for fine-tuning.}



\begin{table}[ht]
    \centering
    \caption{Comparison of CQL with and without $C^4$ on full D4RL locomotion datasets. The module improves the total score without inducing performance degradation.}
    \label{tab:cql-full}
    \resizebox{\textwidth}{!}{
    \begin{tabular}{lccccccccc}
        \toprule
        {Method} & Hop.-m & Hop.-mr & Hop.-me & Half.-m & Half.-mr & Half.-me & Wal.-m & Wal.-mr & Wal.-me \\
        \midrule
        CQL         & 58.5      & 95.0       & \textbf{105.4} & 41.0          & \textbf{45.5}   & 91.6           & 72.5       & 77.2        & \textbf{108.8}       \\
        CQL + $C^4$ & \textbf{85.9} & \textbf{100.7} & 89.4       & \textbf{48.5} & 44.7            & \textbf{91.6} & \textbf{81.8} & \textbf{90.9}    & 108.6      \\
        \bottomrule
    \end{tabular}
    }
\end{table}
% ---------- Figure: Runtime & Sensitivity ----------
\begin{figure}[th]
\centering
\subfigure{\includegraphics[width=0.22\textwidth]{fig/hyparameter/runtime_methods_min.pdf}}
\subfigure{\includegraphics[width=0.22\textwidth]{fig/hyparameter/runtime_plug_min.pdf}}
\subfigure{\includegraphics[width=0.23\textwidth]{fig/parameter/compare_lambda.pdf}}
\subfigure{\includegraphics[width=0.23\textwidth]{fig/parameter/compare_alpha.pdf}}
\caption{\small Wall-clock runtime comparisons, and performance sensitivity to hyperparameters $\lambda$ and $\alpha$.}
\label{fig:runtime}
\end{figure}

\blue{
We further investigate whether $C^4$ acts as a benign addition to standard algorithms when ample data is available. We compare CQL with and without the $C^4$ module across the full D4RL locomotion suite. As shown in Table~\ref{tab:cql-full}, the inclusion of $C^4$ does not hinder performance; on the contrary, it increases the total normalized score from 695.5 to 742.1.
Notably, in tasks where the base algorithm already performs well (e.g., Hopper-medium-expert), $C^4$ maintains competitive performance, while in harder tasks (e.g., Hopper-medium, Walker2d-medium-replay), it provides further gains. This indicates that the gradient-space clustering mechanism naturally scales: as data density increases, the gradient distribution becomes more stable, and our penalty term effectively adjusts without over-regularizing or degrading the policy.}


\begin{figure}[ht]
\centering
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/CQL/Halfcheetah-full-replay.pdf}}
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/CQL/Hopper-medium-expert.pdf}}
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/CQL/Ant-medium-replay.pdf}}
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/CQL/Walker2d-expert.pdf}}
\caption{\small  Performance comparison on CQL vs. (+LN), (+DR3) and (+$C^4$).}
\label{fig:pdf_ablations_CQL}
\end{figure}

\begin{figure}[ht]
\centering
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/TD3BC/Halfcheetah-full-replay.pdf}}
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/TD3BC/Hopper-medium-expert.pdf}}
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/TD3BC/Ant-medium-replay.pdf}}
\subfigure{\includegraphics[width=0.234\textwidth]{fig/ablation/TD3BC/Walker2d-expert.pdf}}
\caption{\small  Performance comparison on TD3BC vs. (+LN), (+DR3) and (+$C^4$).}
\label{fig:pdf_ablations_TD3BC}
\end{figure}

\blue{
We examine the generalization capability of $C^4$ as a plug-in module for established baselines. Using identical training protocols, we compare CQL to CQL augmented with LayerNorm (LN), DR3, and $C^4$ (Fig.~\ref{fig:pdf_ablations_CQL}), and perform a similar comparison for TD3BC (Fig.~\ref{fig:pdf_ablations_TD3BC}). In both algorithm families, incorporating $C^4$ yields the most significant and stable improvements across training, whereas LN and DR3 offer only moderate gains. This demonstrates that $C^4$ effectively isolates the specific variance components that limit performance in standard offline RL algorithms.}


Additionally, extended implementation, benchmark descriptions, experimental details, complete results, and ablations are provided in Appendix \ref{app:expDetails} due to space constraints.


% \input{Appendix/locomotion-table}








==> math_commands.tex <==
%%%%% NEW MATH DEFINITIONS %%%%%

\usepackage{amsmath,amsfonts,bm}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\em (a)}}
\newcommand{\captionb}{{\em (b)}}
\newcommand{\captionc}{{\em (c)}}
\newcommand{\captiond}{{\em (d)}}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}


% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvu{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vtheta{{\bm{\theta}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vf{{\bm{f}}}
\def\vg{{\bm{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sZ{{\mathbb{Z}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\rm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\rm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\rm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\newcommand{\laplace}{\mathrm{Laplace}} % Laplace distribution

\newcommand{\E}{\mathbb{E}}
\newcommand{\Ls}{\mathcal{L}}
\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
\newcommand{\KL}{D_{\mathrm{KL}}}
\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

\DeclareMathOperator*{\argmax}{arg\,max}
\DeclareMathOperator*{\argmin}{arg\,min}

\DeclareMathOperator{\sign}{sign}
\DeclareMathOperator{\Tr}{Tr}
\let\ab\allowbreak

